SoK: Cryptographically Protected Database Search

Protected database search systems cryptographically isolate the roles of reading from, writing to, and administering the database. This separation limits unnecessary administrator access and protects data in the case of system breaches. Since protected search was introduced in 2000, the area has grown rapidly; systems are offered by academia, start-ups, and established companies. However, there is no best protected search system or set of techniques. Design of such systems is a balancing act between security, functionality, performance, and usability. This challenge is made more difficult by ongoing database specialization, as some users will want the functionality of SQL, NoSQL, or NewSQL databases. This database evolution will continue, and the protected search community should be able to quickly provide functionality consistent with newly invented databases. At the same time, the community must accurately and clearly characterize the tradeoffs between different approaches. To address these challenges, we provide the following contributions: 1) An identification of the important primitive operations across database paradigms. We find there are a small number of base operations that can be used and combined to support a large number of database paradigms. 2) An evaluation of the current state of protected search systems in implementing these base operations. This evaluation describes the main approaches and tradeoffs for each base operation. Furthermore, it puts protected search in the context of unprotected search, identifying key gaps in functionality. 3) An analysis of attacks against protected search for different base queries. 4) A roadmap and tools for transforming a protected search system into a protected database, including an open-source performance evaluation platform and initial user opinions of protected search.

==> bookchapter.tex <==
%!TEX root = Book.tex

\section{Secure Search}
\label{sec:securesearch}

The previous section dealt with security and access control for block storage where data can only be retrieved via its unique identifier.  However, in any big data system, users rarely want to retrieve all available data and instead usually only fetch a subset of the available data based on some specified search criteria.  We now switch topics to discuss cryptographic techniques to enable \emph{secure search} allowing for complex, database-style queries to be performed on stored data.

\subsection{Introduction}

\emph{Searchable encryption} refers to a collection of cryptographic techniques that enable a server to perform searches directly over encrypted data.  Most database technologies in use today require a server to be able to read all data contents in order to perform a fast search over it. By contrast, searchable encryption technology permits a server to perform basic database operations directly over encrypted data. Even though the server cannot read the data, it can still return encrypted versions of matching results back to a querier. In summary, searchable encryption technology provides stronger confidentiality and privacy guarantees than those in databases today by separating the roles of providing and accessing data.

There are a myriad of use-cases for this technology in today's interconnected world; we provide just a few examples here. First, in a secure cloud outsourcing scenario, a client can upload files to the cloud and then make searches on the data later, without giving the cloud provider access to read the data. Second, in a secure publish-subscribe system, a broker can properly route messages from many providers to interested subscribers without being able to read the data itself.\footnote{Note that broadcast encryption, described in Section~\ref{sec:broadcast_enc}, achieves a similar goal without using a proxy, but instead requiring providers to know all interested subscribers.}  Third, in a secure email scenario, many senders can send encrypted mail to one receiver, and then the receiver can make searches to her email host to pull only the emails of interest to her without giving the host access to the contents of her emails. Fourth, in a secure database scenario, a data provider can allow multiple clients to search over her data without knowing the locations of data being requested; note here that preventing the data provider from learning the queriers' access patterns (e.g., frequency of requested records and overlaps between sets of records returned in response to different queries) is critical since the provider already knows the contents of her own data, so encryption alone does not suffice here.

Research into searchable encryption has been ongoing for the past 15 years. While there is still work to be done, the current state of this technology is quite usable. First, modern searchable encryption technologies are quite fast: their performance is only about 20\% to 200\% slower than an unprotected search over plaintext data. Second, the searchable encryption works described below cover a large subset of the types of searches typically performed in databases, such as those permitted by the \texttt{where} clause in the Structured Query Language (SQL).  For applications where one is willing to sacrifice a bit in security in exchange for performance, there are alternative searchable encryption schemes that work on top of existing database back-ends (e.g., MySQL and Accumulo) achieving much better performance in exchange for revealing some additional information about the stored data~\cite{PRZB11, cmd}.

\subsection{Definition}

A formal definition of searchable encryption is both complex and ever-changing.  In this chapter, we present an overview of the concepts behind searchable encryption here and then describe some of the complexities in the next section.

\subsubsection{Parties Involved}
The standard model of searchable encryption considers three types of parties: an \emph{owner} who initially possesses the data, a \emph{querier} who wants to learn something about the data, and a \emph{server} who handles the bulk of the storage and processing work. We note that in many scenarios, such as the publish-subscribe and email scenarios above, there may be multiple data owners or queriers.

We note that some scenarios envision only two parties, which we call the querier and server. For instance, the cloud outsourcing scenario above considers a client who acts as both the initial data owner and subsequent querier, and the secure database scenario considers a data owner who does her own server processing.\footnote{The two-party cloud outsourcing scenario in which the owner and querier are the same entity is also used in the model of fully homomorphic encryption, described in detail in Section \ref{sec:he} below.}

We can fit these scenarios into our three-party framework by thinking of them as instances of \emph{collusion}\footnote{Collusion is typically used in cryptography to model a collection of malicious users who are working together, as described in Section \ref{ssec:adversary_model}. But, the same concept applies just as well to the benign setting in which two entities are ``working together'' because they are really the same person.} between two of the three parties: in the cloud outsourcing scenario, the data owner colludes with the querier, and in the second scenario, the data owner colludes with the server.

\subsubsection{Security Guarantees and Limitations} \label{sub:security-guarantees}

In this chapter, we restrict our attention to searchable encryption technologies with \emph{provable} claims about their security.
Here, we overview some of the provable security guarantees provided by searchable encryption technology. First, the querier only learns the contents of records that match her query; she learns nothing about the rest of the owner's dataset, except in some cases its size. Second, the data owner doesn't learn anything about queries being performed on her data. Third, the server performs searches in a relatively oblivious fashion, learning almost nothing about either the data or queries involved.

However, most searchable encryption schemes do reveal or \emph{leak} some information about data and queries to the server. We describe two common leakages that most searchable encryption schemes reveal. First, \emph{search pattern leakage} permits the server to determine if two different queries are identical, even if she cannot learn what the queries are. Second, \emph{access pattern leakage} permits the server to determine which records in the dataset are returned in response to each query, even if she cannot read the records. As a consequence, the server can also determine which records are ``popular'' and being returned in response to many (potentially different) queries.

The precise cryptographic definitions that formalize these security notions have evolved over the years. We describe some of the nuances of these security definitions in Section \ref{sub:sse-survey} and refer interested readers to Bosch et al.'s survey~\cite{Bosch14} for the formal definitions of searchable encryption.


\subsubsection{Trust Requirements}

In order to make provable statements of security like the ones above, searchable encryption schemes (and indeed, all of cryptography) require some pre-conditions to be met: namely, they require users to place their trust in certain aspects of the behavior of other technologies or parties involved in the cryptographic protocol.  Specifically, the searchable encryption schemes commonly rely on assumptions about the allowed adversary behavior, limits on collusion between the involved parties, and computational assumptions for security (See Section~\ref{ssec:adversary_model} for a detailed discussion).

In addition to the above, there are several protocols for secure search that do not require trust in the veracity of computational assumptions but rather in the inability of an adversary to perturb a specialized piece of hardware that performs computations inside of a (hopefully) tamper-proof shell. Put bluntly, these schemes place their trust in an adversary's physical limitations rather than her mathematical ones.  However, as this chapter is focused on software-based solutions, we will only briefly mention one example of such schemes and refer interested readers to the original papers~\cite{SmithS01, BhattacharjeeAGZCCA06, BajajS14}.


\subsection{Survey} \label{sub:sse-survey}

In this section, we first provide a brief history of three important cryptographic prmitives that preceded searchable encryption. Next, we describe some of the initial works on searchable encryption. Finally, we detail several innovations that improve the security of searchable encryption or add new dimensions to the functionality, performance, or security of this technology.

We stress that this section only provides a brief overview of the major thematic advances in searchable encryption technology over the years. We purposely do not delve into all technical details and only present the first few papers that tangibly influenced each theme presented below. For a more detailed, technical review of the (more than 100) research works on searchable encryption, we refer readers to the comprehensive survey by B\"{o}sch \emph{et al} \cite{Bosch14}.

% We note that there are more than 100 papers that tangibly influenced the development of searchable encryption, and we cannot comprehensively survey them all here. Instead, we simply describe the first few papers that make some of the more impactful contributions. For a reasonably comprehensive list of searchable encryption works, we refer readers to \cite{ChaseK10,PappasKVKMCGKB14,FischVKKKMB14,CashJJKRS13,JareckiJKRS13,CashJJJKRS14,PRZB11,Monomi} and all references contained therein.


\subsubsection{History: Precursors to Searchable Encryption}

We begin by describing three cryptographic technologies initially developed in the 1990s that solve related problems. All of these works utilize a two-party setup with a querier and a server. Some of them are better suited to the cloud outsourcing scenario (in which the querier provides the data) and some are better suited to the database setting (in which the server provides the data).

First, \emph{private information retrieval}, or PIR, considers the cloud outsourcing problem in which a data owner outsources her data to an untrusted server and later wants to query for a single record.
While the database contents themselves may be readable in the clear by the server, the querier wants to hide her interests from the server (i.e., which record is being returned in response to a query).
% Intuitively, this can be accomplished by having the server perform a full scan of the database in response to each query.
An important goal in PIR works is to minimize the amount of communication required between the server and querier.
Chor et al.~\cite{ChorKGS98} constructed the first PIR scheme in an information-theoretic model with multiple non-colluding servers.
Shortly thereafter, several works provided PIR under the assumption that certain cryptographic problems are hard \cite{KushilevitzO97,CachinMS99,KushilevitzO00}. We refer interested readers to Gasarch's excellent survey \cite{Gasarch04} for more information about PIR.

Second, Chor et al.~\cite{ChorGN98} introduce \emph{private information retrieval by keywords}. This work introduces the concept of searching (as we think of it today) to the cryptographic literature. Specifically, it uses multiple rounds of PIR to search by keyword rather than by the index (i.e., pointer or unique identifier) of the record that the client wishes to retrieve. Nevertheless, data are still stored unencrypted on the server.

Third, \emph{symmetric private information retrieval}, or SPIR, extends PIR's security guarantees to protect the server as well. Specifically, whereas PIR permits the client to view the entire database, SPIR limits the number of records that a querier may retrieve in response to any query. Hence, SPIR is useful both in the cloud outsourcing scenario and the database scenario, and it can also support multiple queriers securely by using its access controls to restrict each querier to reading only her own data on the server. SPIR was introduced by Gertner et al.~\cite{GertnerIKM00}, though it has its roots in another cryptographic primitive (called oblivious transfer) developed by Rabin in the 1970s \cite{Rabin05}.

Finally, \emph{oblivious random-access memory}, or ORAM, introduces the concept of a server performing keyword searches directly over encrypted data in an \emph{oblivious} fashion; that is, without learning either the contents of any records stored at the server or the access patterns of data returned to the client (such as the simple question ``is this identical to data that the server returned to the client in the past?'').
Goldreich and Ostrovsky's seminal work \cite{GoldreichO96} introduces multiple ORAM techniques, including an asymptotically-optimal logarithmic-time search and a square-root-time search that turns out to be faster in practice \cite{IlievS04}. ORAM has been extensively studied by the cryptographic community since the 1990s, and recent works have substantially improved the server's computational burden \cite{StefanovS13,StefanovDSFRYD13,RenFKSSDD14,DautrichSS14,MoatazMB14,DevadasDFR15,MoatazMB15}.

One performance impediment of ORAM schemes is the large number of rounds of communication that they require between the querier and server. By contrast, most of the searchable encryption works discussed below only require one round of communication. In order to achieve this performance improvement, however, most searchable encryption works reveal some search pattern information to the server.


\subsubsection{Searchable Encryption}

In 2000, Song, Wagner, and Perrig published the seminal work on searchable encryption \cite{SongWP00}. They presented a cryptographic protocol in a two-party setting (with a querier and server) to search over encrypted data that provided the following four properties:
%
\begin{enumerate}

	\item Provable security for encryption: The untrusted server stores ciphertext data that has been encrypted using a semantically-secure encryption scheme (as described in Section \ref{sec:basic-tools}), so the server cannot learn any information about the corresponding plaintexts.

	\item Controlled searching: The untrusted server can only perform searches that have been authorized by the querier. The server cannot make searches on her own.

	\item Hidden queries: Song et al.~support keyword searches. During a query, the server does not learn the keyword. (This concept is later formalized by Goh \cite{Goh03} as ``chosen keyword security'' and defined in a similar style to semantic security.)

	\item Query isolation: While the server does learn which records are returned to the querier, the server learns nothing more about plaintexts than this information.

\end{enumerate}
Additionally, the Song et al.~protocol provides good performance by adhering to a few simple guidelines that subsequent works also follow:
%
\begin{enumerate}

	\item The search protocols are simple and reminiscent of their insecure counterparts.

	\item The scheme relies on faster symmetric-key cryptography rather than slower public-key cryptography. Song et al., in fact, use symmetric-key cryptography exclusively: schemes that follow their lead are collectively referred to as \emph{searchable symmetric encryption}, or SSE. While some of the subsequent works described below do utilize public-key cryptography to provide additional functionality, they often use public-key cryptography as sparingly as possible.

	\item Like most unprotected database search technologies, Song et al.~bolster the performance of queries by pre-computing an \emph{index} mapping keywords to records that match the query. While the bulk of Song et al.'s work is on non-indexed search, this observation foreshadows many of the subsequent works on SSE.

\end{enumerate}
%
After the initial Song et al.~result, a myriad of works improved the functionality, performance, and security of searchable encryption technology.  We now present the various dimensions along which these works improved searchable encryption.  Understanding these dimensions will be important for understanding the state-of-the-art in searchable encryption schemes.
%For ease of exposition, we group these improvements into several categories.

\paragraph{Secure indices:}
Goh \cite{Goh03} formally defines the concept of index-based SSE. We note that indexing induces a performance tradeoff: to achieve faster query throughput, SSE schemes may require a long time to compute the index whenever the database is created or modified. In fact, Song et al.~and Goh do not support efficient database modifications (insertions, updates, or deletions) into their indices due to the difficulty of doing so in a confidential manner (that is, without revealing the desired modification to the server).

Chang and Mitzenmacher \cite{ChangM05} make the valuable observation that indexing provides a clean conceptual separation between two acts that the server must perform: determining the indices of records that match a query and fetching the contents of records at those indices. The first action might require complicated data structures to support sophisticated queries, but the contents of those data structures (i.e., the indices themselves) are small. The second action requires a large data structure to hold record contents but only requires that this data structure support the simplest of queries: a simple pointer-lookup.

With this observation, Chang and Mitzenmacher are able to use standard compression and encryption schemes on the record contents. Chang and Mitzenmacher's observation is utilized in many of the SSE schemes that follow, including all of the works presented in the State of the Art section below (Section \ref{sub:sse-state-of-art}).

\paragraph{Error rates:}
Goh \cite{Goh03} constructs a secure index mechanism whose search time is independent of the number of keywords in the database. To do so, Goh utilizes ``Bloom filters,'' a simple fixed-size data structure that can check for membership in a variable-length set. Goh's indexing mechanism is simple: it builds one Bloom filter per record that includes all of its keywords. Because Bloom filters have a one-sided error, it is possible that the server could return records to the querier that do not actually match the keyword being searched. Subsequent SSE works that utilize Bloom filter technology, such as the Blind Seer \cite{PappasKVKMCGKB14,FischVKKKMB14} scheme discussed in Section \ref{sub:sse-state-of-art} below, also have non-zero false positive rates.

\paragraph{Modifications:}
Due to their separation of searching and file storage, Chang and Mitzenmacher \cite{ChangM05} provide keyword search data structures that are much simpler than those of Song \emph{et al} or Goh. As a result, Chang and Mitzenmacher's index structure supports modifications: insertions, updates, and deletions.  While Chang and Mitzenmacher can only support modifications if they have an \emph{a priori} dictionary or universe of all possible keywords that could be inserted later, subsequent works~\cite{LSDHJ10, PRZB11, KPR12, KP13, CashJJJKRS14, PappasKVKMCGKB14} overcome this restriction and support faster modifications directly over the data structures they use for indexing.

\paragraph{Secure search with multiple queriers:}
Curtmola et al.~\cite{CurtmolaGKO11} formally define SSE with multiple queriers. They do so in two settings: a \emph{non-adaptive} setting in which security is only proved when the adversary must commit to all queries before seeing any responses, and a stronger, \emph{adaptive}, setting in which the adversary is permitted to choose queries based on the responses to prior ones. While adaptively-secure cryptography is preferable for its relevance to real-world usage of SSE, non-adaptive protocols are faster with no known attacks in practice. 

To aid in the multiple-querier setting, Chase and Kamara \cite{ChaseK10} provide an access control mechanism called \emph{controlled disclosure}. This mechanism gives a data owner the ability to grant someone else access to a portion of a large dataset.

\paragraph{Public-key searchable encryption and outsourced SPIR:}
Public-key cryptography enables three-party scenarios (such as the secure publish-subscribe and email scenarios above) in which the server that stores data never has the ability to read or perform searches over it. Boneh et al.~\cite{BonehCOP04} provide the first construction of public-key searchable encryption in which the querier can produce a ``trapdoor'' token that permits the server (non-interactively) to locate all records containing a given keyword without learning anything else. We refer interested readers to Boneh and Waters \cite{BonehW07} for a formal, generic definition of public-key searchable encryption. Many of the works in this space use a relatively novel, powerful, non-standardized cryptographic building block called bilinear groups.

More recently, some of the works described in Section \ref{sub:sse-state-of-art} below attempt to satisfy the security constraints of the three-party scenario (namely, having a server who isn't trusted to learn either the data or queries, as described in Section \ref{sub:security-guarantees} above) while minimizing or removing the use of public-key cryptography in order to improve performance \cite{CashJJKRS13,JareckiJKRS13,CashJJJKRS14,FischVKKKMB14,PappasKVKMCGKB14}. Jarecki et al.~\cite{JareckiJKRS13} refer to this concept as \emph{outsourced SPIR}.

\paragraph{Searching over different data structures:}
Inspired by traditional databases, SSE focuses on the problem of record retrieval via text-based searches. But, just as with the rest of the big data community, encrypted search has progressed beyond this simple setup. Chase and Kamara \cite{ChaseK10} define \emph{structured encryption}, which enables searches over arbitrary structured data such as matrices and graphs. Chase and Shen \cite{ChaseS14a} generalize this notion even further to \emph{queryable encryption}, which permits queries over potentially-unstructured data. Chase and Shen provide one form of queryable encryption: the ability to do a substring search over a large file.

\paragraph{Query expressivity:}
Researchers have steadily increased the expressivity of searchable encryption schemes. Collectively, modern schemes support a large percentage of the selections possible in, for instance, the \texttt{where} clause of the Structured Query Language (SQL).

From the beginning, searchable encryption schemes (and their predecessors in the history section above) supported equality keyword searches such as \texttt{select * where name = Alice}. Researchers subsequently added support for other types of queries, often by finding a new data structure to traverse in a secure fashion. We describe a few of the innovations in data structures below and explain the new query types that they enable.
%
\begin{itemize}

	\item \emph{Boolean queries}: Goh's usage of Bloom filters \cite{Goh03}, as described above, facilitates secure searching for Boolean combinations (i.e., ANDs and ORs) of keywords. The same technique also permits searches for the number of occurrences of a keyword inside a record. Finally, by building a tree of Bloom filters, Goh's technique also facilitates searches for words that occur infrequently in a large dataset, which can be useful for statistical analyses of large datasets. Pappas et al.~\cite{PappasKVKMCGKB14} use a similar Bloom filter technique, and Cash et al.~\cite{CashJJKRS13} support Boolean queries in a different fashion.

	\item \emph{Inequality and range comparisons}: A technique called \emph{order-preserving encryption}, in which the order of ciphertexts matches the order of underlying plaintexts, enables a weak but incredibly fast form of range searches. Research into this technology began in the database community with the work of Agrawal et al.~\cite{AgrawalKSX04}, and it has continued in the cryptographic community with several works that improve the performance and characterize the security limitations of this technology \cite{BoldyrevaCLO09,BoldyrevaCO11,PopaLZ13,MavroforakisCOK15}. On the other end of the spectrum, Boneh and Waters \cite{BonehW07} provide a stronger but slower form of range comparison, subset, and conjunction searches.

	\item \emph{Substrings}: Chase and Shen \cite{ChaseS14a} use a suffix tree data structure to support searches for substrings in a single, large file. Their work operates in the cloud outsourcing two-party scenario.

	\item \emph{Similarity searches}: A few works provide for similarity or fuzzy searches. Park et al.~'s scheme can be used for approximate string matching \cite{ParkKLCZ07}, and Adjedj et al.'s scheme can be used for biometric identification \cite{AdjedjBCK09}.

	\item \emph{Inner products}: A few works provide for searches that involve basic arithmetic operations such as inner product computations \cite{ShenSW09,BoschTHJ12}.

\end{itemize}
%
With support for a broad array of query types, searchable encryption technology is approaching the point of commercial interest \cite{BG14}.

% We note that ORAM technology can also incorporate many of these keyword-based search technologies in a slower but more secure (i.e., with less leakage) fashion than searchable encryption. % \emilysays{But you first need to figure out which IDs to retrieve, which is the hard part, right?}
% Mayank: Commenting out the prior sentence because, while true, I think it adds nothing to the exposition.

%\paragraph{Secure search based on trusted hardware:}
%In this section, we pause to address a fundamentally different way to provide secure search technology through the use of trusted hardware. More specifically, a long line of works have relied upon the usage of secure co-processor hardware platforms such as the IBM 4758 and 4764 PCI cards that are FIPS 140 Level 4 certified for resistance to tampering. These works require parties to have a different type of trust relationship: the querier and data owner must trust that the server performs the sensitive portion of their searches properly on a trusted hardware device.\footnote{We note that some works, like Bouganim and Pucheral \cite{BouganimP02}, consider the use of trusted hardware for the data owner or querier. These works typically use the hardware merely as a safe place to store secret key material, and otherwise perform PIR or software-based searchable encryption in the same manner as we have described in previous sections.}
%
%Smith and Stafford \cite{SmithS01} were the first researchers to propose using trusted hardware for secure searches. They designed and built a server with several IBM 4758 secure co-processors. Following a Map/Reduce-style paradigm, each co-processor computed a portion of the response to a query, and then Smith and Stafford provided a combination step in which these partial answers could be combined in a secure manner to produce the final result.
%
%Smith and Stafford's original scheme was based on the techniques in PIR. By contrast, the next line of works, by Asonov and Freytag \cite{AsonovF02} and Iliev and Smith \cite{IlievS03,IlievS05}, use techniques from ORAM in order to decrease the per-query effort of each secure co-processor at the expense of periodic offline processing. Iliev and Smith use this technique to design a secure LDAP querying service \cite{IlievS03} and, later, a method for secure X.509 certificate exchange \cite{IlievS05}.
%
%Following the same trajectory as the software-based searchable encryption world, the next set of advancements in this technology involve the support of additional query types. Fortunately, query expresssivity is an easier problem to tackle in the trusted hardware space, since these systems are able to execute the same computations as unprotected data search technology; the trick here is not so much in performing the computations in a cryptographically-secure manner but rather in determining which small subset of those computations are ``sensitive'' and must be performed inside the secure hardware.
%
%To provide some concrete examples of research into query expressivity: Agrawal et al.~\cite{AgrawalAKL06} implement secure JOINs, Bhattacharjee et al.~\cite{BhattacharjeeAGZCCA06} perform data mining and analysis in the secure co-processor, and Bajaj and Sion \cite{BajajS14} provide a full relational database whose data structures and query processing methods are split into secure pieces run on an IBM 4764 and insecure components running on commodity hardware.
%
%We conclude with a note on the scalability of this technology. Bajaj and Sion estimate the cost of computatations, storage, and networking in both small-scale and large-scale (``the cloud'') computing environments. They conclude that, at scale, computation inside secure processors is only 2-4$\times$ more costly than computation in small-scale insecure enterprises, and thus orders of magnitude faster than any cryptographic operation.

\paragraph{Performance and scale improvements:}
Finally, we examine two methods utilized to improve the performance and scalability of searchable encryption: pre-processing and parallelization.

First, Freedman et al.~\cite{FreedmanIPR05} developed a technique to save on online query processing time by performing some pre-processing work between the querier and server (a technique that is also used in ORAM schemes).
% Freedman et al's work also introduces the concept of privacy for the data owner: that the querier is limited to learning records that match her query, as described in the Security Guarantees section above.
Second, Kamara and Papamanthou~\cite{KP13}, Cash et al.~\cite{CashJJJKRS14}, and Pappas et al.~\cite{PappasKVKMCGKB14} discover opportunities for parallelization, both within a single query's execution and between several queries that are executed concurrently. With these performance improvements, these works are able to handle significantly larger databases, with the latter two works scaling to achieve good performance on terabyte-sized datasets. We discuss these two works, along with other modern, usable searchable encryption techniques, next.


% Mayank: Commenting out Ariel's stuff so they can be maintained separately from my contributions.
% Arkady:  I am including this as an include to avoid having to copy and paste stuff.  This should also make it easier for Mayank to make changes without having to depend on any other files in SVN
\input{securesearch_stateoftheart}

==> leakage.tex <==
%!TEX root = main.tex

\subsection{Communicating the Impacts of Leakage} 
\label{sec:crypto-security-leakage-informal}

\mv{Perhaps we should add a question asking performers about their
opinions on the possible side-channel attacks to which their system may be
vulnerable.}

In this section, we provide several questions for any protected database
designer to answer about the security of their cryptographic protocols, including
the implications and consequences of their system's leakage. We offer these
questions because cryptographic security definitions are (1) inherently
worst-case, (2) imprecise when it comes to leakage, and (3) are difficult to communicate to non-experts.
 As such, we purposely pose the questions in this section informally, and they should be answered
answer them informally; 
The answers to these questions will help communicate the unique features and benefits of your system.

Unless otherwise stated, the questions of this section are meant to apply to all
roles (as defined in \secref{sec:entities}).  We present two sets of questions, in the first designers are asked to consider the general behavior of their system.  In the second, we describe a specific database and ask designers to consider leakage in this example.  The goal of this example is to familiarize designers with the process of considering leakage and data simultaneously.

\subsubsection{General Questions}
\ben{say something before starting the enumeration}
\begin{enumerate}
\item Describe, at a high level, any leakage that is inherent in your
core protocol.  Describe what specific leakage this results in for each of the
implemented query types, especially for query types not implemented in Phase 1.
 
\item \label{enum:three-qs} Describe a ``worst-case scenario'' for your
	system. That is, describe an example database and set of queries
	for which your leakage is particularly harmful. In particular:
  \begin{enumerate}
  \item Exactly what leaks, as precisely as possible, during initialization,
	updates, and queries. Describe which party or parties are being
	compromised by this leakage.
  \item Why you believe this leakage is damaging to the overall
    security of the system.
  \item How many queries can be made, and how many records can be
    returned by the database, before the leakage becomes problematic
    in this scenario.
  \end{enumerate}


\item Conversely, describe a ``best-case scenario'' for your
  system. That is, describe an example database and set of
  queries for which your leakage is particularly benign. For this scenario,
	please answer the same three questions posed in Question \ref{enum:three-qs}.

\item Describe a realistic database and set of queries for
  which your leakage is reasonable and would not substantively harm
  users of the system. Again, answer the three questions posed above in Question
	\ref{enum:three-qs} for this scenario.
  
\item Does your system have a mechanism for mitigating future leakage?
Is there a ``reset'' mechanism that allows you to separate
leakage before and after in such a way that they are somehow
uncorrelated. (including, but not limited to, a re-initialization of the entire
system)? If so: 
\begin{enumerate}
\item What is the ``reset'' algorithm, how costly is it, how often
would you recommend running it, and can you amortize its cost by executing it in
an incremental or continuous fashion?
\end{enumerate}

\item Many cryptographic models assume for
simplicity that every field (and thus, every record) is of fixed
length. This question considers the effect of variable-length data
structures used by your privacy-preserving database management system.
%
	\begin{enumerate}
					\item Does your system involve any variable-length data structures?
					(An example of this would be the storage of \texttt{VARCHAR}s
					in MySQL.)

					\item What additional leakage is provided to each party due to the
					variable-length records? Answer this question with respect to all roles in the system.

					% \item Which security properties in Section \ref{sec:crypto-security-leakage}
					% are violated due to this leakage?
	\end{enumerate}

\item What information about policy decisions is revealed to each role in the system?
\begin{enumerate}
\item
Specifically, what restrictions on
(the composition of) policies, queries and databases need to be imposed for your
protocol to satisfy any formal security guarantees?
\ben{I'm not sure I understand this phrasing}
\end{enumerate}

\item \label{enum:software-bits-security}
For this question \emph{only}, you should consider the implementation of
your crypto protocols in the software,
rather than the generic capabilities of your cryptographic protocols.
Describe all of the cryptographic protocols that you use in
your software, such as all encryption routines and hash functions. Then, explain
the key length(s) that are used in your software and justify that they
consistently provide the same level of security.
\ben{Im not sure this fits, is there a better place for it?}

\end{enumerate}

\subsubsection{Use Case Based Questions}
In this section, we describe a general corpus of real-world data and ask designers to think about the impact of leakage for that corpus.  The corpus is as follows: the database and queries are drawn
  (roughly speaking) from the population of the United
  States.\footnote{The authors wish to emphasize that this example was
    crafted independently of any known use-case, and was based solely
    upon the availability of publicly-available real-world data. }  This corpus can be generated using our evaluation platform (described in \secref{sec:eval platform}).
%  At a high level: consider a database of 100,000 elements,
%  independently and identically distributed according to a probability
%  distribution built to crudely reflect the population of the United
%  States.
%   As before, answer the following questions: 
%  
%\begin{enumerate}
%\item What does leakage reveal about records present and absent?
%\item What does leakage reveal about queries made or not made?
%\end{enumerate}

We first provide a detailed description of the database and accompanying queries and then describe the questions.
%To aid in answering these questions, we provide a complete description of the database and queries.  


  \begin{table}
  \begin{centering}
    \begin{tabular}{|l|l|l|}\hline
      Field & Type & Size (bytes) \\ \hline
      Last Name & CHAR & 50 \\
      First Name & CHAR & 50 \\
      Gender & ENUM & 1 \\
      Age & INT & 1 \\
      State & ENUM & 1 \\ \hline
%      Words & Char & 100\\ \hline
    \end{tabular}
    \caption{Census Based Example Use Case.}
    \label{tab:census data}
    \end{centering}
  \end{table}
  
  \paragraph{Database Contents}   The database schema is presented in \tabref{tab:census data}. Assume that
  the database contains 100,000 entries.  It is possible for the database to contain more
  than one record with a given set of values. Such duplicate records
  will count as multiple individual records.\footnote{One can imagine that
  records are indexed by unique keys, so two records with identical
  values will receive distinct indexes, thus distinguishing them in
  the database.}  The database is distributed as follows: last name,
  state, age and words are all selected independently of all other
  values in the record. First name and gender are selected jointly,
  but independently of all other values in the record.
  \begin{itemize}
  \item Last names are drawn from the distribution induced by the 1000
    most common last names as calculated by the 1990 United States
    Census~\cite{last-name-census}.\footnote{Specifically, they are drawn from the top 1,000
      names, 
      where the probability of any name is computed as the ratio of
      the names's `frequency in percent' (column 2) to the `cumulative
      frequency in percent' (column 3) of the 1000th name (`Vang').  Both male and female first names are selected the same methodology.}
  \item Gender and first name are selected jointly.
    \begin{itemize}
    \item With probability .5, the gender will be `female' and the
      first name selected according to the distribution of the top
      1000 female names of the 1990 United States
      Census~\cite{first-name-female-census}.
    \item With probability .5, the gender will be `male' and the first
      name selected according to the distribution of the top 1000 male
      names of the 1990 United States Census~\cite{first-name-male-census}.
    \end{itemize}
  \item Age and state are each (individually) is distributed according
    to the distribution induced by the 1990 United States
    Census (\cite[Table 13, Column 1]{general-pop-census} and \cite[Table 16, 1990]{state-census} respectively).\footnote{
%    Age is distributed according to `General
%      Population Characteristics: United States'
%      (\url{http://www.census.gov/prod/cen1990/cp1/cp-1-1.pdf}), Table
%      13, Column 1 (`All persons: total'). 
      For the purposes of this
      question, assume that all persons of age `105 years and over'
      are of age 105 years. 
%      State is distributed according to `1990
%      Census of Population and Housing: Population and Housing Unit
%      Counts'
%      (\url{http://www.census.gov/prod/cen1990/cph2/cph-2-1-1.pdf}),
%      Table 16, Column 1990, for individual states and District of
%      Columbia.
      }
%  \item The words field holds five words, separated by a space
%    character, selected independently according to the frequency of
%    English words in Project Guttenberg.\footnote{That is, five words
%      are chosen independently and identically according to the
%      frequencies of the 10,000 most frequent words in Project
%      Guttenberg as computed by Connel MacKenzie in 2006
%      (\url{http://en.wiktionary.org/wiki/Wiktionary:Frequency_lists/PG/2006/04/1-10000}).}\footnote{The `Words' field will be used, later, to ask about leakage from
%  queries of type `keyword' and `stemming.'}
  \end{itemize}
  
  \ben{I want to move most of these footnotes to citations, very tough to read}

\paragraph{Queries} Queries using the following process:
  \begin{itemize}
  \item Choose a random bit $b$ uniformly from $\{0,1\}$.
  \item If $b=0$, generate a query which matches at least one record
    in the database according to the following:
    \begin{itemize}
    \item Randomly and uniformly select a record from the database
      (treating duplicates as individual records, as above).
    \item Uniformly select two
      attributes from \{first name, age, state, gender\} to be
      removed.
    \item The resulting query is a conjunction over equality queries
      over the three remaining attributes using the values for those
      attributes in the chosen record.
    \end{itemize}
  \item If $b=1$ generate a query which matches no
    records in the database, according to the following procedure:
    \begin{itemize}
    \item Select a new record from the database-generation distribution
      described above.
    \item Uniformly select two
      attributes from \{first name, age, state, gender\} to be removed.
    \item The resulting query is a conjunction over equality queries
      over the three remaining attributes using the values for those
      attributes in the sampled record.
    \item If this query matches any records in the database, discard
      it and repeat until a query is generated which matches no
      records in the database.
    \end{itemize}
  \end{itemize}

For schemes that do not support conjunctions, we recommend creating inserting all triples of possible field combinations as keywords.  Since last name is included in all queries this is only $12$ possible combinations.
\ben{Mayank revise this description. Shortened commented out description below.}
% (We note that these queries ignore the `Words' field. That field
%  will be considered below. Also, we note that performers who do not
%  support conjunctions can still support this scenario. Because it is
%  guaranteed that all queries will provide exact values for three
%  fields---one of which will be last name---it is known that there
%  will be exactly 12 possible query structures. Any given record can
%  be stored under 12 `pointers': one for each query which could match
%  it. This induces an expansion on database size and execution time,
%  but this question does not require any analysis of performance.)

\paragraph{Questions}
Consider the following informal questions.  Estimates and arguments are encouraged provided they illuminate the revelant system characteristics.
  \begin{enumerate}
  \item How can your leakage be interpreted (if possible) in
      terms of names, ages, etc. of persons present or absent in the
      database?
  \item How many queries can occur before your leakage reveals
      that the database contains particular records? In particular describe, 
      \begin{enumerate}
      \item For all roles, consider the leakage observable by that role over
    $n$ queries. In some systems, this leakage may allow the party to
    conclusively identify a particular record (with specific values
    for all five attributes) that is in the database but has not
    matched any query. More specifically, any given value of $n$ will
    map to a probability (over the randomness of the database and the
    queries) that the role in question can make such a statement,
    about some record, with absolute certainty. For each role, and
    for your system, how high do you believe $n$ can grow before this
    probability becomes 10\%? 50\%?  90\%?
    \end{enumerate}
  \item How many queries can occur before your leakage reveals
      that the database does \emph{not} contain particular records? Answer in the same format as the previous question.
%      \begin{enumerate}
%      \item
%    That is, reconsider the probability of the previous question, but
%    now about the likelihood that the given party can identify some
%    record (with specific values for all five attributes) which is
%    conclusively \emph{not} in the database. For each party, and for
%    your system, how high do you believe $n$ can grow before this
%    probability becomes 10\%? 50\%? 90\%?
%    \end{enumerate}
  \item How many queries can occur before your leakage reveals
      which queries have been made? Answer in the same format as the previous questions.
%      In particular describe,
%\begin{enumerate}
%\item For each role, consider
%    the leakage observable by that role over $n$ queries. In some
%    systems, this leakage may allow the party to conclusively identify
%    a particular query (identifying the three attributes used and the
%    specific values for all three attributes) that was made. More
%    specifically, any given value of $n$ will map to a probability
%    (over the randomness of the database and the queries) that the
%    party in question can make such a statement, about some query,
%    with absolute certainty. For each party, and for your system, how
%    high do you believe $n$ can grow before this probability becomes
%    10\%? 50\%? 90\%?
%    \end{enumerate}
  \item How many queries can occur before your leakage reveals
      which queries have \emph{not} been made? Answer in the same format as the previous questions.
      \end{enumerate}
      
%      \begin{enumerate}
%  \item \textbf{What about queries with conjunctions, keywords, and
%      stemming?} Consider the following new distribution of queries:
%
%  \begin{itemize}
%  \item First, choose a random bit $b$ uniformly from $\{0,1\}$.
%  \item If $b=0$, generate a query which matches at least one record
%    in the database according to the following procedure:
%    \begin{itemize}
%    \item Randomly and uniformly select a record from the database
%      (treating duplicates as individual records, as above).
%    \item Select, uniformly from all possible combinations, one
%      attribute from \{first name, age, state, gender\} to be
%     retained.
%    \item Select one work from that record's `words' field.
%    \item The resulting query is the conjunction: (last name = that
%      from chosen record) and (relevant attribute = retained
%      attribute) and (stem of chosen word as keyword of `words'
%      field).
%    \end{itemize}
%  \item If $b=1$, on the other hand, generate a query which matches no
%    records in the database, according to the following procedure:
%    \begin{itemize}
%    \item Select a new record from the database-generation distribution
%      described above.
%    \item Select, uniformly from all possible combinations, one
%      attributes from \{first name, age, state, gender\} to be retained.
%    \item Select one work from that record's `words' field.
%    \item The resulting query is the conjunction: (last name = that
%      from chosen record) and (relevant attribute = retained
%      attribute) and (stem of chosen word as keyword of `words'
%      field). 
%   \item If this query matches any records in the database, discard
%      it and repeat until a query is generated which matches no
%      records in the database.
%    \end{itemize}
%  \end{itemize}
%
%  How do your answers to the above four questions change if queries
%  are selected from this new distribution?
%
%\end{enumerate}
%%\end{enumerate}
%
%
%%%% Local Variables: 
%%%% mode: latex
%%%% TeX-master: "ROE.tex"
%%%% End: 


==> methodology.tex <==
%!TEX root = main.tex

\section{Systematization Methodology}
\label{sec:sys method}
%In this section, we discuss our approach to distilling the vast number of potential database operations to a much smaller core set of basis functions. %This approach borrows heavily from our experience developing standards for databases and developing hardware accelerated math libraries.
%From the 1970s to the 1990s, the Structured Query Language (SQL) and relational data model dominated the database community (and arguably, still do). The relational model was used for large variety of applications; it was \emph{the solution} for data that needed to be indexed and queried using a predetermined API (SQL).  The security community identified protected search emerged as an area of interest at this time.  Naturally, most protected search systems were designed to meet the needs of SQL style applications.
Since 2000, DBMSs have significantly diversified. 
Databases are often customized and designed for specific workloads or use cases.  
%While reproducing SQL and relational database functionality is not an easy task for the security community, it was a relatively static task when compared to the rate at which new systems are being developed.  
Creating a protected version of database takes time - how will the community keep up if a new database paradigm is introduced every five years?  Our approach is to identify base operations that are likely to be useful across multiple database paradigms (presented in \tabref{tab:db classes}).  Using this identification, protected search development can then be split into three components: 1) create protected versions of base queries (\secref{sec:custom}) and 2) create methods to combine queries to support complex searches that do not depend on the underlying implementation (\secref{sec:extending func}) 3) adding support for additional DBMS functionality such as rules and performance tuning (\secref{sec:queries-to-systems}).  

%The question of what functions to optimize or secure can be a difficult one. On one hand, it is easy to look at some of the most common operations that users perform and attempt to secure those operations. On the other hand, if there is a basis or core set of operators that can be composed to create a much wider set of operations, one could secure those core operators and build more complex (and perhaps useful) operators out of those. Our group has extensive experience with performance optimization for database and compute systems. Our approach in such cases is to leverage a relatively small set of operators that can be effectively optimized and build more complex operators out of these operators. Our belief is that analytics and queries change over time and it is better to optimize a core set of operators, which we refer to as a base operations, that can be used to create new operators as the time comes. We believe that this approach taken to optimizing hardware and software systems can also be utilized by cryptographers. By securing a smaller set of core functionality that can then be used to create more complicated operators, we hope that the challenge of providing secure operations in database systems as operations continue to change at a rapid pace can be more tractable. When a particular operation or query becomes popular or widely used, it can then be optimized.
%
%In many cases, the database community is realizing the value of such basis functions in order to optimize performance (hardware manufacturers, for example, can now optimize a small set of basis operations). However, these basis functions can be used just as easily to distill down to a core set of operations for cryptographers. Many database systems (or the tools used to access data within them) already adhere to such a principles. Rather than developing a complete list of functions, E.F Codd, in his seminal paper on relational databases, described six basis functions that could be used to construct a rich language. He showed how a complicated query could be represented as a combination of these basic functions.  For graph databases as another example, standardization groups have been working on expressing complex graph analytics using simple linear algebraic operations (similar to the BLAS supported by most current processors) that can be optimized by the hardware or software community. We understand that there may be some debate on the exact definition of these basis functions. However, we believe that the operations we will describe closely resemble most possible basis functions. Protected basis functions can then be used to construct a wide variety of protected operations. However, in many cases, a user/application may need to use a particular operation only. In such cases, using only the basis functions (while functional) may not perform efficiently and optimized secure operations may be necessary.
%
%Thus, we believe that it is important for protected search system designers to simultaneously work on two tasks: 1) developing secure versions of database basis functions and 2) optimizing particular operations (a combination of the base queries) as the need arises.  To understand how to address these two problems, we first review different types of unprotected databases.

%In addition to understanding whether a protected search system offers the right usability vs. security tradeoff, one must know if it supports the data model needed by your application.  To begin to answer this question, we first provide a brief introduction on the types of DBMSs.

%\paragraph{The state of unprotected databases}
%
%SQL was built on relational algebra as described by Codd in 1970~\cite{codd1970relational}.  Codd presented a succinct \emph{basis} of functions sufficient to build a relational database: select, project, union, set difference, Cartesian product, and rename.  Complex queries could by \emph{combining} operations from this small basis.  For nearly thirty years, SQL and relational data models became the dominant DBMS solution. SQL style DBMSs still occupy a large fraction of the data management market.
%
%In the mid-2000s, Chang et al., proposed the Google BigTable \cite{chang2008bigtable} database capable of rapidly ingesting the vast quantities of data being indexed from the internet. Their design had no schema and spurred the Not only SQL (NoSQL) movement. Now a multi-billion dollar industry, there are many NoSQL databases.  Many other styles of database engines fall into the NoSQL category such as graph databases~\cite{angles2008survey}, object databases, document stores, etc. Typically, NoSQL databases excel at rapid data ingest or provide intuitive data models that align with future computation or data being stored.\ay{Elaborate here.}
%
%NewSQL is a new wave of database management technologies databases that couple strong correctness guarantees with the high performance of NoSQL databases~\cite{grolinger2013data}. These systems typically rely on improved hardware capabilities or re-architected systems or limited data models to provide high performance access with strong guarantees.

%These three classes of database engines have their relative merits and are currently used by a large number of users. %Further, there has been a greater bifurcation in the number of languages to express database analytics and SQL is no longer the only database management language.

%In the near future, we expect federated databases~\cite{carey1995towards,elmore2015demonstration}, which employ multiple database backends to intelligently and efficiently answer queries, to become the norm.
%In this system, a client's query will be transformed by a \emph{query planner} that understands each database backend.  This query planner transform the client's query into \emph{basis} operations of each backend technology.  It then estimates the time to execute the query on each technology and executes the query on the fastest technology.  Note that while all databases follow the framework of a fast optimized basis and reduction of complex queries to this basis, each database technology has a different basis.
%This creates a moving target for protected search designers, leaving a divide between protected search systems and databases in use.



==> outline.tex <==
%!TEX root = main.tex

\section{Outline of New Draft}
\label{sec:outline}

\begin{enumerate}
\item Introduction
\begin{enumerate}
\item What is protected search?  
\item Why does it matter? Ground swell of work in both academia and now commercial (we cover commercial offerings in Section I-A)
\item What is in scope for this work?  What is out of scope?
\item What is our goal in this paper? 
\item How are databases built?  Use the example of relational algebra.  How does a database administrator choose their database back end?  Introduce the concept of query planning
\item Protected Search Systems Today
\item ORAM, Token, PPE
\item Why is choosing a protected search system more complicated?  
\item These systems have imperfect security to achieve performance targets
\item This means, in addition to finding a system that supports your query load, you also need to understand what protections will be provided by that scheme.  The query planner's task is also more complicated now.  It needs to balance efficiently executing the query and understanding the security impacts.  
\item This leads to our systemization methodology.  We first define security and note that most systems are proved security with respect to similar security definitions.  Security differences only become apparent in systems imperfections, which are generally called leakage.  This is data that is unintentionally revealed to a party that should not learn it.
 We first classify approaches as described above.  We then classify approaches on the basic operations that are supported by their cryptography.  Like traditional database systems, protected search systems natively support some operations and then combine these operations to provide a wider range of queries.  
 \item Leakage systemization
 \item This only gives a snapshot of current systems.  We describe current and projected database paradigms and their corresponding basis functions.  We use this view to identify fundamental operations that are unknown or immature in the cryptographic literature.  We also use this view to identify opportunities to implement systems in novel ways that have not yet been done in the literature.
 \item Applications differ in two basic ways: security needs and functionality (different types of DBs are build for different queries, different with a protected search system is if functionality wasn't designed it may not work as opposed to being slow)
 \item Need to talk about security at a level accessible to a DB user
\end{enumerate}
\item Modeling protected search systems, how to understand security?
\item Protected Search Systems (Table I) 
\begin{enumerate}
\item Creating the closure of functionality.  (Table II) 
\end{enumerate}
\item Interpreting security, what does leakage mean? (Table III) 
\item Database trends, important research problems (Table IV) 
\item Where do we go from here (usability study, evaluation platform)
\item Conclusion
\end{enumerate}

==> rel_work.tex <==
%!TEX root = main.tex


\subsection{Related cryptographic problems}
\label{sec:rel problems}

In this section we discuss cryptographic primitives that are related to protected database search.  We discuss six primitives: 1) private information retrieval, 2) symmetric private information retrieval, 3) oblivious RAM 4) fully homomorphic encryption 5) multi-party computation and 6) functional encryption.  The first three tools solve similar problems (and are used as components in protected database search constructions), the last three tools are currently too inefficient to solve the problem (and some have lower bounds on achievable efficiency).  We discuss more below:

1) In \emph{private information retrieval}, or PIR, a data owner outsources her data array to an untrusted server and later wants to query for a single record.
While the data array itself may be readable in the clear by the server, the querier wants to hide her interests from the server (i.e., which element is being returned).
% Intuitively, this can be accomplished by having the server perform a full scan of the database in response to each query.
An important goal in PIR works is to minimize the amount of communication required between the server and querier.
Chor et al.~\cite{FOCS:CGKS95} constructed the first PIR scheme in an information-theoretic model with multiple non-colluding servers.
Shortly thereafter, several works provided PIR under the assumption that certain cryptographic problems are hard \cite{FOCS:KusOst97,EC:CacMicSta99,EC:KusOst00}. We refer interested readers to Gasarch's excellent survey \cite{Gasarch04} for more information about PIR. 

PIR fails to meet the requirements of protected search in two ways; data contents are not protected from the server, and the  searching functionality is not sufficient to perform complex searches. 

Chor et al.~\cite{EPRINT:ChoGilNao98} introduce \emph{private information retrieval by keywords}. This work introduces the concept of searching (as we think of it today) to the cryptographic literature. Specifically, it uses multiple rounds of PIR to search by keyword rather than by the index (i.e., pointer or unique identifier) of the record that the client wishes to retrieve. %Nevertheless, data are still stored unencrypted on the server and query utility is still limited.

2) \emph{Symmetric private information retrieval}, or SPIR, extends PIR's security guarantees to hide contents from the server. Specifically, whereas PIR permits the client to view the entire database, SPIR limits the number of records that a querier may retrieve in response to any query. \ben{I really don't understand this sentence.  How does hiding contents limit what the client can retrieve?  Couldn't they only get one record before?} Hence, SPIR can support multiple queriers securely by using its access controls to restrict each querier to reading only her own data on the server. SPIR was introduced by Gertner et al.~\cite{STOC:GIKM98} but has roots in oblivious transfer~\cite{Rabin05}. While SPIR does improve the security against the searcher, data's contents still remains unsecured against the server and there are similar limitations on query functionality. 
\ben{this whole paragraph is tough for me, maybe I just don't understand SPIR}

3) \emph{Oblivious random-access memory}, or ORAM~\cite{STOC:Goldreich87}, allows a server to perform index retrieval over encrypted data obliviously; that is, without learning either the contents of any records stored at the server or the access patterns of data returned to the client (such as the simple question ``is this identical to data that the server returned to the client in the past?'').
%Goldreich and Ostrovsky's seminal work \cite{GoldreichO96} introduces multiple ORAM techniques, including an asymptotically-optimal logarithmic-time search and a square-root-time search that turns out to be faster in practice \cite{IlievS04}. 
ORAM has been extensively studied by the cryptographic community since the 1990s, and recent works have substantially improved the server's computational burden \cite{SP:SteShi13,EPRINT:SDSFRY13,EPRINT:RFKSSv14,DautrichSS14,FC:MMBC15,TCC:DDFRSW16,EPRINT:MoaBlaMay15}. However, even with increased performance, ORAM does not support searches beyond simple index retrieval, which does not support the utility needed for encrypted database search. 
\ben{ORAM out of the box does not allow key word searches, it allows index retrieval.  If there is a simple transform I don't know about, I'd like to mention it here.  I don't want to expand the definition of ORAM to be keyword searchable.}

4) \emph{Fully Homomorphic Encryption}, or FHE, is a type of public-key encryption that allows anyone to compute arbitrary functions over data while it is encrypted without decrypting it or learning anything about it. Many encryption schemes are naturally homomorphic in one operation (either addition or multiplication) \cite{C:ElGamal84,EC:Paillier99,Rabin78,RivShaAdl78} but not both. In 2009, Gentry \cite{STOC:Gentry09} demonstrated the first encryption scheme that provides $eval$ operations for an unbounded number of both additions and multiplications by \emph{bootstrapping}. 

Recent work has increased the number of $eval$ operations possible before bootstrapping, eliminating bootstrapping altogether, or making bootstrapping more efficient \cite{ITCS:BraGenVai12,PKC:GenHalSma12}. 
\ben{I want to expand this citation list a bit, its incomplete}
 Bootstrapping is the most expensive part of homomorphic evaluation, and reducing the frequency with which it needs to be done greatly increases evaluation efficiency. While this does push FHE towards the realms of practicality, the techniques are still too slow to be used in traditional encryption search setting. 
 \ben{can we include a recent estimate?  maybe from Nigel's paper?}

5) Secure \emph{Multi-party Computation} (MPC) allows multiple people to perform arbitrary distributed computation on their private data without revealing their data. MPC protocols exist for any computable function and for any number of parties.  It can broadly be broken into the classes; two-party \cite{FOCS:Yao82b}, where efficient implementations use garbled boolean circuits, 
\ben{is this too broad a generalization?  do all 2PC techniques fall into this class?} and multi-party computation \cite{STOC:BenGolWig88,STOC:GolMicWig87}, which relies on polynomials. 
\ben{can we say anything about the state of art?  also I don't think its fair that all MPC is based on polynomials}
Recently, MPC compilers \cite{CCS:HKSSW10,CCS:BenNisPin08,SP:SHSSK15} allow generic programs to be represented as MPC interactions, however, generic MPC remains too slow to be practical for use in encrypted search.

6) \emph{Functional Encryption} (FE) allows certain computations to be performed on encrypted data while allowing the data owner to restrict both who can compute on the ciphertext and what computations may be done. Sahai and Waters proposed the concept of functional encryption as a generalization of attribute-based encryption~\cite{EC:SahWat05}. General constructions have been proposed based on multilinear maps~\cite{FOCS:GGHRSW13}. However, there are some very strong limitations to the types of FE schemes that can be constructed in terms of efficiency, security, and generality~\cite{TCC:BonSahWat11}. FE is currently considerably slower than FHE and based on less standard assumptions.  In fact only one implementation FE currently exists \cite{} and that has proven to be too slow for any practical application. 

\ben{Arkady can you revise this paragraph?}



==> sse_today.tex <==
%!TEX root = main.tex


%\subsection{Protected Search Systems Today}
\subsection{Protected Search Approaches}
In this subsection, we describe three high-level approaches that are used to provide protected search.  The guiding principle of the first approach is to use an unprotected database server.  This approach only modifies how data is stored on this server and how the client prepares queries.  We call this approach \ppe or \shortppe.

Alternatively, one can also modify how the server performs queries, making the server is ``aware'' it is performing protected search.  We call this approach \sse or \shortsse. We also identify a third approach that is a subset of \shortsse that provides stronger security.  This approach uses techniques from \oram and we refer to it as \shortoram.  We make this distinction because \shortsse and \shortoram schemes provide currently different levels of protection based on the attacks from the literature that we discuss in \secref{sec:leakage-attack}.
We provide a short overview of each approach:

\paragraph{\shortppe} The goal of a \shortppe approach is to produce an ``encrypted'' set of records that still allows the server to use its standard indexing mechanism.  Special types of encryption called \emph{property-preserving encryption} preserve various properties of the plaintext such as equality and ordering without leaking additional information.

%For example, consider a dataset containing social security numbers, where we want to allow a \emph{client} to return a record if they match a particular social security number (SSN).  Rather than inserting the unprotected keyword `123 45 6789' into the database, the client \emph{deterministically encrypts}~\cite{C:BelBolONe07} the record obtaining $\mathtt{Enc}('123 45 6789')$.  The encryption key is held by the client and never revealed to the server.  When querying for this record, the client recreates the encryption and queries the database for all records whose SSN is $\mathtt{Enc}('123 45 6789')$.

%Various cryptographic approaches have been developed that preserve different \emph{properties} of the plaintext and thus allow different searching functionality (for example, order preserving encryption~\cite{EPRINT:BCLO12} allows the database to execute range queries).  Popa et al. described the first system to integrate these techniques into a protected search system~\cite{CACM:PRZB12}.  In general this approach is able to replicate most database management system (DBMS) functionality with a performance overhead of under 30\%~\cite{CACM:PRZB12}.  This approach is used by most of the commercial products listed above and has been extended to NoSQL key-value stores~\cite{kepner2014computing,gadepally2015computing}.

However, this backwards compatibility comes at a cost to security.  The encryption techniques must leak some information to the server about the entire dataset for it to answer queries.  In the case of deterministic encryption, the server learns which records are equal (and thus an unlabeled histogram of the data).

\paragraph{\shortsse} The second approach, \sse, also modifies the database server.  This approach creates protected versions of traditional database indices that are designed to be traversed jointly by the querier and the server.  The provider can help the server prepare indices in such a way that they reveal minimal information in the absence of queries.  This approach has more flexibility in what is leaked to the server.  In general, \shortsse schemes have less leakage than \shortppe schemes at the cost of reduced functionality and performance.  \emily{Is it true that \shortsse schemes have reduced functionality compared to \shortppe? We know how to do equality and range with PPE but not more expressive queries.} Most \shortsse schemes leak some information to the server based on how the indices are traversed (access patterns) and some statistical information on the data that can be learned by analyzing the indices.

%In turn, these systems reduce the amount of leakage provided to the server.  While each approach differs in what is revealed (see \secref{sec:security}), the guiding principle is that nothing should be learned about a record before that record is queried.\ay{I would not claim this, I do not think any \shortsse schemes actually achieve this.  All leakage reveals something about the distribution of other values in the DB.}  Continuing the SSN example, the server may be able to tell if a record with the same SSN is returned in multiple queries.  This is in contrast to \shortppe where the server learns which records have the same SSN even if no queries are made.\ay{Be careful here, CryptDB leaks nothing until a query is made.}

\paragraph{\shortoram}
\shortoram uses the same setup as \shortsse.  It takes a more conservative view on what should be revealed to the server.  In particular, It hides repeated retrieval of the same record.  

==> test.tex <==
%!TEX root = main.tex

\subsection{Evaluation Platform}
\label{sec:eval platform}

\mv{Make sure that the BSD license claim is correct.}

We developed an evaluation platform as part of IARPA's Security and Privacy Assurance Research (SPAR) program in order to evaluate the integrity and performance of several protected databases \cite{%
FCW:CFGPPW14,CrescenzoCMP14,CrescenzoS14,CrescenzoG15,% ACS
SP:PKVKMC14,SP:FVKKKM15,% Columbia/Bell Labs
C:CJJKRS13,NDSS:CJJJKR14,ESORICS:FJKNRS15,% IBM
RSA:IKLO16% Stealth
}. Our platform has been open-sourced with a BSD license, and it is available at \url{https://github.com/mitll-csa/sparta}. We remark that our platform cannot validate any confidentiality or privacy claims.  We separately designed formal verification tools that can do so \cite{PetcherM15a,PetcherM15b}.

\mv{Cite also Alley's work if/when it gets published.}

\subsubsection{Components}

At a high level, our platform encompasses three components: a data and query generator \cite{HamlinH14}, an orchestrator for the test \cite{VariaPHHHPRYC15}, and a post-test automatic report generator \cite{FCW:VarYakYan15}. These components respectively provide rapid data generation, rapid environmental reconfiguration, and rapid status reporting. Additionally, they combine together to provide repeatable, end-to-end automation and integration of the entire evaluation process. The platform was used to test SQL-style databases, yet it was designed with reusability and extensibility in mind so that it may be generalized to evaluate other types of databases.
\ariel{I am comfortable saying that the code is generalizable to other SQL-style databases, but for at least the data/query gen, it is \emph{not} generalizable for other database types}

Before testing, our data generator built artificial but realistic-looking data corresponding to people's names, addresses, birthdays, etc.~based upon data from the US Census Bureau \cite{Census_PUMS,Census_surnames} and Project Gutenberg \cite{Gutenberg} in a repeatable fashion \cite{WCBRRC10}. It can produce 100 million rows of synthetic data with 20 integer, date, string, and binary blob fields in about 9 hours on a 12 core machine. Concurrently, our integrated query generator tool can generate queries with fine-grained control over several characteristics that can affect performance, such as the number of results returned or query type.

During testing, our Ansible-like~\cite{ansible} custom test orchestrator drives a database system under test (SUT). Specifically, it installs all SUT software components (typically one per role) along with our platform artifacts on different machines within the testbed environment, distributes queries to the querier or modifications to the provider as governed by a test script file, and then captures and saves the integrity and performance metrics described below into a SQLite~\cite{hipp2007sqlite} database for later dissection by people and by our automatic report generator tool. In order to treat the SUT as a black box, we specify an interface by which developers can distribute and instantiate the components of the SUT without testing, and then we compose our platform components around them as needed.

After testing, our automatic report generator converts the evaluation results from a machine-friendly SQLite database into a human-friendly LaTeX report, complete with tables and graphs (like Fig.~\ref{fig:histogram}) generated by NumPy \cite{numpy}. In short, it provides the ``Experimental Results'' section of a report for a new protected database technology. Moreover, its automation provides agility during the design of a software package, enabling rapid visualization and identification of anomalies and bugs.
\ariel{Do we want to say anything about the run time of the report generator?}

\begin{figure}[t]
\centering
% \fbox{\includegraphics[scale=.5]{included-files/SPAR-rr-ui-abridged.png}}
Todo
\caption{Sample histogram produced by our automatic report generator.}
\label{fig:histogram}
\end{figure}


\subsubsection{Metrics gathered}
\label{sub:metrics}

We measure the integrity of query responses, database modifications, and policy checks by measuring their \emph{precision} (the fraction of observed behaviors that are correct) and \emph{recall} (the fraction of correct outcomes that are observed) \cite{precision_recall}. To make these metrics well-formed, we must decide whether to measure them in isolation or while other database operations are ongoing. In fact, there is a rough mapping between terminology between the cryptographic and database communities: of the four properties that collectively form ACID compliance, \emph{consistency} and \emph{durability} roughly correspond to the integrity of a single operation, whereas \emph{atomicity} and \emph{isolation} capture integrity properties that must hold under concurrent composition of database commands.

Additionally, our platform captures several performance characteristics of queries and modifications. We stress upfront that the performance of a large, stateful system like a database depends on many features. For example, the performance of queries can depend on:
%
\begin{itemize}
\item Environmental characteristics: the amount of CPU cores and RAM dedicated to each role, along with the behavior of the network connecting them (for a sufficiently slow connection, the cryptographic protocols effectively become `free').
\item Size of the database: number of tables, number of rows and columns, etc.
\item Query type (e.g., the number of alternations in a boolean query and the number of clauses at each level).
\ariel{There was definitely more to the query types than the alterations or number of clauses, we had 9 different atomic types}
\item Response profile: the number of records returned by the entire query and also by each of its individual components (e.g., for a conjunction of 2 clauses, the number of records each clause individually would return).
\item Policy: The presence and complexity of the policy assurance mechanism applied to the query.
\end{itemize}
%
Therefore, our query generator has the sophistication to vary queries along each of these dimensions independently, so that we may capture and graph cross-sections of the performance hull. \ariel{Query generation only covered about 2 of these, and datagen gets another 2, I think this is the wrong place for this point and it should be moved up into the query/data generation paragraph} Furthermore, our resulting metrics for the latency and throughput of queries and modifications are not displayed as single numbers, but rather percentile histograms (see Fig.~\ref{fig:histogram}) that show the variation in performance across the full distribution of queries tested. \ariel{Didn't quite understand this sentence}

To capture all of these metrics, our platform enables arbitrary interleaving of operations. It accepts a test script containing any combination of queries, modifications, and policy updates. It may operate in one of two extremes, latency mode (each command completes before the next is executed) or throughput mode (commands are fed as fast as a SUT can accept them), or anything in between them (the next command is executed after a fixed time delay or when the SUT reports completion of the prior command). Additionally, each script may operate in isolation or with another script executing concurrently in another thread; hence, we may test for atomicity and isolation errors by running (potentially related) queries and modifications in parallel and observing the outcomes. Finally, to understand the impact of our machine specs on the test results, we systematically capture the CPU, RAM, disk, and network usage on all machines using \texttt{collectl} \cite{collectl} and \texttt{tcpdump} \cite{tcpdump}, and we vary the network's latency and throughput using \texttt{tc} \cite{tc}.

\mv{My citations for software packages are rather sparse. Someone may want to edit them in the future.}

